12.2-GHz methanol maser MMB follow-up catalogue - II. Longitude range 186 to 330 degrees

We present the second portion of a catalogue of 12.2-GHz methanol masers detected towards 6.7-GHz methanol masers observed in the unbiased Methanol Multibeam (MMB) Survey. Using the Parkes radio telescope we have targeted all 207 6.7-GHz methanol masers in the longitude range 186 to 330 degrees for 12.2-GHz counterparts. We report the detection of 83 12.2-GHz methanol masers, and one additional source which we suspect is thermal emission, equating to a detection rate of 40 per cent. Of the 83 maser detections, 39 are reported here for the first time. We discuss source properties, including variability and highlight a number of unusual sources. We present a list of 45 candidates that are likely to harbor methanol masers in the 107.0-GHz transition.

==> PaxHeader/12GHz_Cat_II_s.tex <==
14 gid=286778
14 uid=270925
20 ctime=1342058800
20 atime=1342058800
38 LIBARCHIVE.creationtime=1340250615
24 SCHILY.dev=234881026
22 SCHILY.ino=8527118
18 SCHILY.nlink=1

